Towards Making Deep Transfer Learning Never Hurt

Transfer learning have been frequently used to improve deep neural network training through incorporating weights of pre-trained networks as the starting-point of optimization for regularization. While deep transfer learning can usually boost the performance with better accuracy and faster convergence, transferring weights from inappropriate networks hurts training procedure and may lead to even lower accuracy. In this paper, we consider deep transfer learning as minimizing a linear combination of empirical loss and regularizer based on pre-trained weights, where the regularizer would restrict the training procedure from lowering the empirical loss, with conflicted descent directions (e.g., derivatives). Following the view, we propose a novel strategy making regularization-based Deep Transfer learning Never Hurt (DTNH) that, for each iteration of training procedure, computes the derivatives of the two terms separately, then re-estimates a new descent direction that does not hurt the empirical loss minimization while preserving the regularization affects from the pre-trained weights. Extensive experiments have been done using common transfer learning regularizers, such as L2-SP and knowledge distillation, on top of a wide range of deep transfer learning benchmarks including Caltech, MIT indoor 67, CIFAR-10 and ImageNet. The empirical results show that the proposed descent direction estimation strategy DTNH can always improve the performance of deep transfer learning tasks based on all above regularizers, even when transferring pre-trained weights from inappropriate networks. All in all, DTNH strategy can improve state-of-the-art regularizers in all cases with 0.1%--7% higher accuracy in all experiments.

==> app.tex <==

\begin{table*}[!h]
    \centering
        \caption{Classification Accuracy Comparison with Source task \textbf{ImageNet} \cite{deng2009imagenet}.}
    \begin{tabular}{c||cc||cc}
    \hline
   Target Datasets & $L^2$-SP & \TheName\ ($L^2$-SP) & KnowDist &\TheName\ (KnowDist) \\
    \hline
    Caltech 256 (30)  & $80.81 \pm 0.11$ & $\bm{81.01 \pm 0.06}$ &  $79.35 \pm 0.21$ & $\bm{80.50 \pm 0.27}$\\
    Caltech 256 (60) & $83.69 \pm 0.09$ & $\bm{84.14 \pm 0.08}$ & $82.93 \pm 0.08$ & $\bm{83.27 \pm 0.4}$\\
     MIT Indoors 67 & $ 75.11 \pm 0.43 $ & $\bm{77.46 \pm 0.29}$ & $78.05 \pm 0.32$ & $\bm{78.77 \pm 0.31}$\\
     Flowers 102 & $88.96 \pm 0.21$ & $\bm{90.68 \pm 0.31}$ & $90.43 \pm 0.4$& $\bm{90.91 \pm 0.4}$\\
     CIFAR 10 & $93.30 \pm 0.16$ & $\bm{96.41 \pm 0.11}$ & $96.43 \pm 0.08$ & $\bm{96.57 \pm 0.2}$ \\
    \hline
    \end{tabular}
    \label{tab:1}
\end{table*}

\begin{table*}[!h]
    \centering
        \caption{Classification Accuracy Comparison with Source task \textbf{Places 365} \cite{zhou2017places}.}
    \begin{tabular}{c||cc||cc}
    \hline
    Target Databsets & $L^2$-SP & \TheName\ ($L^2$-SP) & KnowDist &\TheName\ (KnowDist) \\
    \hline
     Caltech 256 (30) & $62.48 \pm 0.32$ & $\bm{66.44 \pm 0.16}$ & $65.31 \pm 0.43$ & $\bm{65.50 \pm 0.17}$\\
     Caltech 256 (60) & $66.99 \pm 0.20$ & $\bm{73.32 \pm 0.1}$ & $72.8 \pm 0.22$ & $\bm{73.18 \pm 0.24}$\\
     MIT Indoors 67 & $84.09 \pm 0.09$ & $\bm{84.19 \pm 0.07}$ & $83.29 \pm 0.42$ & $\bm{84.40 \pm 0.41}$\\ 
     Flowers 102 & $77.66 \pm 0.13$ & $\bm{84.11 \pm 0.06}$ & $83.50 \pm 0.26$ & $\bm{84.12 \pm 0.56}$\\
     CIFAR 10 & $89.78 \pm 0.05$ & $\bm{90.85 \pm 0.11}$ & $94.96 \pm 0.05$ & $\bm{95.02 \pm 0.13}$\\
    \hline
    \end{tabular}
    \label{tab:2}
\end{table*}

\begin{table*}[!h]
    \centering
        \caption{Classification Accuracy Comparison with Source task \textbf{Stanford Dogs 120} \cite{khosla2011novel}.}
    \begin{tabular}{c||cc||cc}
    \hline
    Target Datasets & $L^2$-SP & \TheName\ ($L^2$-SP) & KnowDist &\TheName\ (KnowDist) \\
    \hline
     Caltech 256 (30)  & $80.59\pm 0.16$ & $\bm{80.86 \pm 0.02}$ & $78.94 \pm 0.27$ & $\bm{79.55 \pm 0.30}$\\
     Caltech 256 (60) & $83.44 \pm 0.23$ & $\bm{83.84 \pm 0.08}$ & $82.73 \pm 0.26$ & $\bm{82.85 \pm 0.27}$\\
     MIT Indoors 67  & $74.64 \pm 0.07$ & $\bm{76.46 \pm 0.22}$ & $76.36 \pm 0.19$ & $\bm{76.74 \pm 026}$\\ 
     Flowers 102  & $88.14 \pm 0.06$ & $\bm{89.98 \pm 0.04}$ & $89.86 \pm 0.07$ & $\bm{90.29 \pm 0.34}$\\
     CIFAR 10  & $94.16 \pm 0.10$ & $\bm{96.39 \pm 0.08}$ & $96.11 \pm 0.53$ & $\bm{96.41 \pm 0.18}$\\
    \hline
    \end{tabular}
    \label{tab:3}
\end{table*}

==> data.tex <==
\begin{table*}
    \centering
        \caption{Classification Accuracy Comparison with Source task \textbf{ImageNet} \cite{deng2009imagenet}.}
    \begin{tabular}{c|c|ccccc}
    \hline
   Target Datasets & Source & $L^2$ & $L^2$-SP & \TheName($L^2$-SP) & KnowDist &\TheName(KnowDist) \\
    \hline
    Caltech 256 30 & ImageNet & $78.92 \pm 0.13$ & $80.81 \pm 0.11$ & $\bm{81.01 \pm 0.06}$ &  $79.35 \pm 0.21$ & $80.50 \pm 0.27$\\
    Caltech 256 60 & ImageNet & $82.68 \pm 0.2$ & $83.69 \pm 0.09$ & $\bm{84.14 \pm 0.08}$ & $82.93 \pm 0.08$ & $83.27 \pm 0.4$\\
     Stanford Dogs 120 & ImageNet &  $80.51 \pm 0.17$ & $84.15 \pm 0.16$ & $\bm{84.21 \pm 0.08}$ & $80.87 \pm 0.2$ & $81.50 \pm 0.25$\\
     MIT Indoors 67 & ImageNet & $76.73 \pm 0.77$ & $ 75.11 \pm 0.43 $ & $77.46 \pm 0.29$ &$78.05 \pm 0.32$ & $\bm{78.77 \pm 0.31}$\\
     Flowers 102 & ImageNet & $90.24 \pm 0.31$ & $88.96 \pm 0.21$ & $90.68 \pm 0.31$ & $90.43 \pm 0.4$& $\bm{90.91 \pm 0.4}$\\
     CIFAR 10 & ImageNet & $96.35\pm 0.4$ & $93.30 \pm 0.16$ & $96.41 \pm 0.11$ & $96.43 \pm 0.08$ & $\bm{96.57 \pm 0.2}$ \\
    \hline
    \end{tabular}
    \label{tab:1}
\end{table*}

\begin{table}[]
    \centering
            \caption{Classification Accuracy without Deep Transfer Learning under the Same Settings}
    \begin{tabular}{c|c}\hline
        Datasets &  Accuracy \\\hline 
       Caltech 256 (30)  & \\
       Caltech 256 (60)  & \\
 %      Stanford Dogs 120    & \\
       MIT Indoors 67 & \\
       Flowers 102  &   \\
       CIFAR 10  & \\\hline
    \end{tabular}
    \label{tab:original}
\end{table}

\begin{table}[]
    \centering
            \caption{Observation: If Deep Transfer Learning Hurts?}
    \begin{tabular}{cc|c}\hline
        Source & Target &  Hurt? \\\hline 
        ImageNet & Caltech 256 (30)  & \\
        ImageNet &Caltech 256 (60)  & \\
        ImageNet & MIT Indoors 67 & \\
        ImageNet &  Flowers 102  &   \\
        ImageNet &  CIFAR 10  & \\\hline
        Place365 & Caltech 256 (30)  & \\
        Place365 & Caltech 256 (60)  & \\
        Place365 & MIT Indoors 67 & \\
        Place365 &  Flowers 102  &   \\
        Place365 &  CIFAR 10  & \\\hline
        Standford Dog 120 & Caltech 256 (30)  & \\
        Standford Dog 120 &Caltech 256 (60)  & \\
        Standford Dog 120 & MIT Indoors 67 & \\
        Standford Dog 120 &  Flowers 102  &   \\
        Standford Dog 120 &  CIFAR 10  & \\\hline
    \end{tabular}
    \label{tab:original}
\end{table}


\begin{table*}
    \centering
        \caption{Classification Accuracy Comparison with Source task \textbf{Places365} \cite{zhou2017places}.}
    \begin{tabular}{c|c|ccccc}
    \hline
    Database & Source & $L^2$ & $L^2$-SP & \TheName($L^2$-SP) & KnowDist &\TheName(KnowDist) \\
    \hline
     Caltech 256 30 & Places365 & $65.38 \pm 0.42$ & $62.48 \pm 0.32$ & $\bm{66.44 \pm 0.16}$ & $65.31 \pm 0.43$ & $65.50 \pm 0.17$\\
     Caltech 256 60 & Places365 & $73.13 \pm 0.20$ & $66.99 \pm 0.20$ & $\bm{73.32 \pm 0.1}$ & $72.8 \pm 0.22$ & $73.18 \pm 0.24$\\
     MIT Indoors 67 & Places365 & $82.64 \pm 0.16$ & $84.09 \pm 0.09$ & $84.19 \pm 0.07$ & $83.29 \pm 0.42$ & $\bm{84.40 \pm 0.41}$\\ 
     Flowers 102 & Places365 & $83.77 \pm 0.68$ & $77.66 \pm 0.13$ & $84.11 \pm 0.06$ & $83.50 \pm 0.26$ & $\bm{84.12 \pm 0.56}$\\
     CIFAR 10 & Places365 & $89.35 \pm 0.59$ & $78.90 \pm 0.142$ & $90.85 \pm 0.11$ & $\bm{94.96 \pm 0.05}$ & $94.96 \pm 0.13$\\
    \hline
    \end{tabular}
    \label{tab:2}
\end{table*}

\begin{table*}
    \centering
        \caption{Classification Accuracy Comparison with Source task \textbf{Stanford Dogs} \cite{khosla2011novel}.}
    \begin{tabular}{c|c|ccccc}
    \hline
    Database & Source & $L^2$ & $L^2$-SP & \TheName($L^2$-SP) & KnowDist &\TheName(KnowDist) \\
    \hline
     Caltech 256 30 & Stanford Dogs & $65.38 \pm 0.42$ & $62.48 \pm 0.32$ & $66.44 \pm 0.16$ & & \\
     Caltech 256 60 & Stanford Dogs & $73.13 \pm 0.20$ & $66.99 \pm 0.20$ & & & \\
     MIT Indoors 67 & Stanford Dogs & $82.64 \pm 0.16$ & $84.09 \pm 0.10$ & & & \\ 
     Flowers 102 & Stanford Dogs & $83.77 \pm 0.68$ & $77.66 \pm 0.13$ & $84.11 \pm 0.06$ & & \\
     CIFAR 10 & Stanford Dogs & $89.35 \pm 0.59$ & $78.90 \pm 0.142$ & $90.85 \pm 0.11$ & & \\
    \hline
    \end{tabular}
    \label{tab:3}
\end{table*}

==> record_wrs.tex <==
\begin{table*}
    \centering
    \begin{tabular}{c|c|ccccc}
    \hline
    Database & Source & $L^2$ & $L^2-SP$ & $L^2-SP$(DTNH) & $fm-SP$ &$fm-SP$(DTNH) \\
    \hline
    Caltech 256 30 & ImageNet & $78.92 \pm 0.13$ & $80.81 \pm 0.11$ & $\bm{81.01 \pm 0.06}$ &  $79.35 \pm 0.21$ & $80.50 \pm 0.27$\\
    Caltech 256 60 & ImageNet & $82.68 \pm 0.2$ & $83.69 \pm 0.09$ & $\bm{84.14 \pm 0.08}$ & $82.93 \pm 0.08$ & $83.27 \pm 0.4$\\
     Stanford Dogs 120 & ImageNet &  $80.51 \pm 0.17$ & $84.15 \pm 0.16$ & $\bm{84.21 \pm 0.08}$ & $80.87 \pm 0.2$ & $81.50 \pm 0.25$\\
     MIT Indoors 67 & ImageNet & $76.73 \pm 0.77$ & $ 75.11 \pm 0.43 $ & $77.46 \pm 0.29$ &$78.05 \pm 0.32$ & $\bm{78.77 \pm 0.31}$\\
     Flowers 102 & ImageNet & $90.24 \pm 0.31$ & $88.96 \pm 0.21$ & $90.68 \pm 0.31$ & $90.43 \pm 0.4$& $\bm{90.91 \pm 0.4}$\\
     CIFAR 10 & ImageNet & $96.35\pm 0.4$ & $93.30 \pm 0.16$ & $96.41 \pm 0.11$ & $96.43 \pm 0.08$ & $\bm{96.57 \pm 0.2}$ \\
    \hline
    \end{tabular}
    \caption{Comparing top-1 accuracy using data augmentation for three regularization methods and their DTNH version, source task is \textbf{ImageNet} \cite{deng2009imagenet}.}
    \label{tab:1}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|c|ccccc}
    \hline
    Database & Source & $L^2$ & $L^2-SP$ & $L^2-SP$(DTNH) & $fm-SP$ &$fm-SP$(DTNH) \\
    \hline
     Caltech 256 30 & Places365 & $65.38 \pm 0.42$ & $62.48 \pm 0.32$ & $\bm{66.44 \pm 0.16}$ & $65.31 \pm 0.43$ & $65.50 \pm 0.17$\\
     Caltech 256 60 & Places365 & $73.13 \pm 0.20$ & $66.99 \pm 0.20$ & $\bm{73.32 \pm 0.1}$ & $72.8 \pm 0.22$ & $73.18 \pm 0.24$\\
     MIT Indoors 67 & Places365 & $82.64 \pm 0.16$ & $84.09 \pm 0.09$ & $84.19 \pm 0.07$ & $83.29 \pm 0.42$ & $\bm{84.40 \pm 0.41}$\\ 
     Flowers 102 & Places365 & $83.77 \pm 0.68$ & $77.66 \pm 0.13$ & $84.11 \pm 0.06$ & $83.50 \pm 0.26$ & $\bm{84.12 \pm 0.56}$\\
     CIFAR 10 & Places365 & $89.35 \pm 0.59$ & $78.90 \pm 0.142$ & $90.85 \pm 0.11$ & $\bm{94.96 \pm 0.05}$ & $94.96 \pm 0.13$\\
    \hline
    \end{tabular}
    \caption{Comparing top-1 accuracy using data augmentation for three regularization methods and their DTNH version, source task is \textbf{Places365} \cite{zhou2017places}.}
    \label{tab:2}
\end{table*}
